Extracting Label-specific Key Input Features for Neural Code Intelligence Models

The code intelligence (CI) models are often black-box and do not offer any insights on the input features that they learn for making correct predictions. This opacity may lead to distrust in their prediction and hamper their wider adoption in safety-critical applications. In recent, the program reduction technique is widely being used to identify key input features in order to explain the prediction of CI models. The approach removes irrelevant parts from an input program and keeps the minimal snippets that a CI model needs to maintain its prediction. However, the state-of-the-art approaches mainly use a syntax-unaware program reduction technique that does not follow the syntax of programs, which adds significant overhead to the reduction of input programs and explainability of models. In this paper, we apply a syntax-guided program reduction technique that follows the syntax of input programs during reduction. Our experiments on multiple models across different types of input programs show that the syntax-guided program reduction technique significantly outperforms the syntax-unaware program reduction technique in reducing the size of input programs. Extracting key input features from reduced programs reveals that the syntax-guided reduced programs contain more label-specific key input features and are more vulnerable to adversarial transformation when renaming the key tokens in programs. These label-specific key input features may help to understand the reasoning of models' prediction from different perspectives and increase the trustworthiness to correct classification given by CI models.

==> resources/models.tex <==
\begin{table}
    \begin{center}
        \caption{Performance of the CI models on test set.}
        \def\arraystretch{1.23}
        \label{table:ci_models}
        \resizebox{0.95\columnwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|}
            \hline
            \textbf{Model} & \textbf{Dataset} & 
            \textbf{Precision} & \textbf{Recall} & \textbf{$F_1$-Score} \\ \hline 
            \hline
            \ctv & \multirow{2}{*}{\JL} & 45.17 & 32.28 & 37.65 \\ \cline{1-1} \cline{3-5}
            \cts & & 64.03 & 55.02 & 59.19 \\ \hline 
        \end{tabular}%
        }
    \end{center}
\end{table}


==> settings.tex <==
\section{Implementation}

To implement and evaluate our approach, we study two well-known code intelligence models (\ctv and \cts), a popular code intelligence task (\mnp) and one commonly used programming language dataset (\JL) with different type input programs. However, our approach can be applicable to other models, tasks, and programming languages.


\subsection{Task:}
We use the popular code intelligence task: method name prediction (\mnp \cite{allamanis2015suggesting}) in this study. This task is commonly used by researchers in the code intelligence domain for various applications such as code summarization \cite{allamanis2015suggesting,allamanis2016summarization}, representation learning \cite{alon2019code2vec,alon2019code2seq}, neural testing \cite{kang2019generalizability,yefet2020adversarial,rabin2021generalizability}, feature extraction \cite{rabin2021sivand,wang2021demystifying}, and so on \cite{allamanis2018bigcode, allamanis2019duplication}.
In this \mnp task, a model attempts to predict the name of a method from its body. For example, given the following code snippet: ``\texttt{void f(int a, int b) \{int temp = a; a = b; b = temp;\}}'', a model aims to predict the method's name as ``\texttt{swap}''.





\subsection{Model:}
We use two well-known \ci models for \mnp task: \ctv~\cite{alon2019code2vec} and \cts~\cite{alon2019code2seq}. Both models use paths from abstract syntax trees (AST) to encode a program.
\begin{itemize}
    \item \ctv. This model extracts a bag of path-context from the AST of the program where each path-context includes a pair of terminal nodes and the corresponding path between them. The model learns embeddings of these path-contexts during training and uses an attention mechanism to aggregate multiple path-contexts to a single code vector. The code vector is used as a representation of the program for making a prediction.
    \item \cts. This model also extracts a bag of path-context from the AST of the program but it sub-tokenized each path-context. The \cts model uses a bi-directional LSTM to encode paths node-by-node, and another LSTM to decode a target sequence one-by-one.
\end{itemize}
Using \texttt{JavaExtractor} of \ctv and \cts models, we extract and preprocess the bag of path-contexts from Java files. For example, given a sample expression: ``\texttt{tempVar = 0;}'', a path-context by \ctv is: ``\texttt{tempVar, <NameExpr ↑ AssignExpr ↓ IntegerLiteralExpr>, 0}'' and a path-context by \cts is: ``\texttt{temp|var, NameExpr | AssignExpr | IntegerLiteralExpr, 0}''.

\subsection{Dataset}
For the \mnp task, we use the \JL dataset \cite{alon2019code2seq}. This dataset contains a total of $9,500$ Java projects from GitHub, where $9,000$ projects are for the training set, $200$ projects for the validation set, and $300$ projects for the test set. Using training set and validation set, we train both the \ctv and \cts models. Table ? summarizes the performance characteristics of these models.

\subsection{Input Types}
The dataset from GitHub is often imbalanced and contains different sizes and frequencies of input programs. Therefore, to evaluate the effectiveness of our approach, we choose different type of input programs from \JL test set.

\begin{itemize}
    \item Frequent Methods: We randomly sample a total of $100$ input programs from the most occurring method names.
    \item Rare Methods: We randomly sample a total of $100$ input programs from the least occurring method names.
    \item Smaller Methods: We randomly sample a total of $100$ input programs that contains less than $10$ lines of code.
    \item Larger Methods: We randomly sample a total of $100$ input programs that has around $100$ lines of code.
\end{itemize}

